A Peer to Peer Protocol for Online Dispute Resolution over Storage Consumption

In bilateral accounting of resource consumption both the consumer and provider independently measure the amount of resources consumed by the consumer. The problem here is that potential disparities between the provider's and consumer's accountings, might lead to conflicts between the two parties that need to be resolved. We argue that with the proper mechanisms available, most of these conflicts can be solved online, as opposite to in court resolution; the design of such mechanisms is still a research topic; to help cover the gap, in this paper we propose a peer--to--peer protocol for online dispute resolution over storage consumption. The protocol is peer--to--peer and takes into consideration the possible causes (e.g, transmission delays, unsynchronized metric collectors, etc.) of the disparity between the provider's and consumer's accountings to make, if possible, the two results converge.

==> eptcsdata.tex <==
\providecommand{\event}{M.H. ter Beek (Ed.): Young Researchers Workshop\\
on Service-Oriented Computing 2009 (YR-SOC'09).
}
\providecommand{\volume}{2}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{3}
\providecommand{\eid}{1}

